PrivilegedDreamer: Explicit Imagination of Privileged Information for Rapid Adaptation of Learned Policies

Numerous real-world control problems involve dynamics and objectives affected by unobservable hidden parameters, ranging from autonomous driving to robotic manipulation, which cause performance degradation during sim-to-real transfer. To represent these kinds of domains, we adopt hidden-parameter Markov decision processes (HIP-MDPs), which model sequential decision problems where hidden variables parameterize transition and reward functions. Existing approaches, such as domain randomization, domain adaptation, and meta-learning, simply treat the effect of hidden parameters as additional variance and often struggle to effectively handle HIP-MDP problems, especially when the rewards are parameterized by hidden variables. We introduce Privileged-Dreamer, a model-based reinforcement learning framework that extends the existing model-based approach by incorporating an explicit parameter estimation module. PrivilegedDreamer features its novel dual recurrent architecture that explicitly estimates hidden parameters from limited historical data and enables us to condition the model, actor, and critic networks on these estimated parameters. Our empirical analysis on five diverse HIP-MDP tasks demonstrates that PrivilegedDreamer outperforms state-of-the-art model-based, model-free, and domain adaptation learning algorithms. Additionally, we conduct ablation studies to justify the inclusion of each component in the proposed architecture.

==> tables/dreamer-hyperparameters-table.tex <==
\begin{table}[h]
\begin{tabular}{|l|l|}
\hline
\multicolumn{2}{|c|}{\textbf{Dreamer Hyperparameters}} \\ \hline
\textbf{Parameter} & \textbf{Value} \\ \hline
Replay buffer size & $5 \text{ x } 10^{5}$ \\ \hline
$\gamma$ discount & 0.99 \\ \hline
Batch size & 1024 \\ \hline
Learning rate (encoder, decoder, and LSTM) & $10^{-4}$ \\ \hline
Learning rate (actor) & $2 \text{ x } 10^{-4}$ \\ \hline
Learning rate (critic) & $8 \text{ x } 10^{-5}$ \\ \hline
Hidden layers (all networks) & [400, 400, 400, 400] \\ \hline
Hidden dimension (actor and critic) & 1024 \\ \hline
Discount $\lambda$ & 0.95 \\ \hline
Gradient clipping threshold & 100 \\ \hline
Imagination horizon & 15 \\ \hline
LSTM hidden dimension & 64 \\ \hline
\end{tabular}
\end{table}

==> tables/ppo-hyperparameter-table.tex <==
\begin{table}[h]
\begin{tabular}{|l|l|}
\hline
\multicolumn{2}{|c|}{\textbf{PPO Hyperparameters}} \\ \hline
\textbf{Parameter} & \textbf{Value} \\ \hline
Learning rate & $3 \text{ x } 10^{-4}$ \\ \hline
Steps per update & 2048 \\ \hline
Batch size & 64 \\ \hline
$\gamma$ discount & 0.99 \\ \hline
GAE $\lambda$ & 0.95 \\ \hline
Clip range & 0.2 \\ \hline
Gradient clipping threshold & 0.5 \\ \hline
\end{tabular}
\end{table}

==> tables/rma-hyperparameters-table.tex <==
\begin{table}[h]
\begin{tabular}{|l|l|}
\hline
\multicolumn{2}{|c|}{\textbf{RMA Hyperparameters}} \\ \hline
\textbf{Parameter} & \textbf{Value} \\ \hline
Encoder shape & [256, 128] \\ \hline
History size & 25 \\ \hline
Train size & 100000 \\ \hline
Learning rate & 0.004 \\ \hline
Activation & ELU \cite{Clevert2015} \\ \hline
\end{tabular}
\end{table}

==> tables/sac-hyperparameters-table.tex <==
\begin{table}[h]
\begin{tabular}{|l|l|}
\hline
\multicolumn{2}{|c|}{\textbf{SAC Hyperparameters}} \\ \hline
\textbf{Parameter} & \textbf{Value} \\ \hline
Replay buffer size & $10^6$ \\ \hline
Seed steps & 5000 \\ \hline
Initial temperature & 0.1 \\ \hline
$\gamma$ discount & 0.99 \\ \hline
Batch size & 1024 \\ \hline
Learning rate (all networks) & $10^{-4}$ \\ \hline
Hidden layers (actor and critic) & [1024, 1024] \\ \hline
Critic $\tau$ & 0.005 \\ \hline
\end{tabular}
\end{table}
